Multi-Version Conflict Notion

This paper introduces the useful notion of Multi-Version Conflict notion.

==> algo.tex <==
\section{MVC Algorithm}
\label{sec:algo}

\subsection{Result obtained so far}
As a part of this research, we developed a MVC(Multiversion Conflict) algorithm which satisfies Conflict Opacity. This algorithm has developed for Multiversion STMs based on multiversion conflicts.

\textbf {MVC algorithm works as follows:-}
\begin{enumerate}
\item \textbf{Read rule:} An operation $r_i(x)$ can read from the most previous closest write. If addition of Commit-read conflict edge to the $MVCG(H)$ will form a cycle then it will read from the next-previous closest write and so on. It ensures read always succeeds. In other words, any read operation can reads from at least one of the available version that will never form a cycle in the graph.
\item \textbf{Write rule:} Transaction $T_i$ writes into local memory.
\item \textbf{Commit rule:} If it is a read-only transaction, then always commits. If it is not, then for every try-to-commit, if it is founded conflict and the corresponding conflict edge will form a cycle in the graph then try-to-commit operation will be rejected and transaction will abort otherwise succeeds.

\end{enumerate}

\subsection{Data Structures}

\subsection{Pseudo code}

\subsection{Correctness of MCN}


==> conc.tex <==
\section{Conclusion}
\label{sec:conc}

This paper studied the concise description of multiversion conflict opacity. This also described the technique for garbage collection to reduce the memory consumption of multi-version STMs. This paper has used MCN algorithm. Then with the help of MCN algorithm we showed that if a schedule generated by this algorithm is multiversion conflict opaque then the graph will be acyclic. In terms of acyclic graph construction, this paper gives a new definition for multiversion conflict notion. Here we have also proved that even of the garbage collection the history will be still acyclic.

==> gar.tex <==
\section{Garbage Collection}
\label{sec:gar}
One of the practical application of Multi-versioned STM is garbage collection. The earlier STM such as Versioned boxes~\cite{CachRito:tran1:2006} consists of a fixed number of old object versions which has not been longer used, increases the overload on the system. In this model, we are maintaining the entire history. So in this context garbage collection means delete a transaction from history. In other words, if we want to delete a transaction, we have to delete it from a history.

\textbf{When a transaction can be deleted?}

The STM system will automatically delete the transaction when the following conditions are satisfied:

\cmnt {
\begin{enumerate}
\item STM system can delete a transaction $T_i$ only if all the live set transactions of $T_i$ will be terminated.
\end{enumerate}

\begin{algorithm}  [!ht]
\scriptsize
\label{alg:20} 
\caption{STM $clean\_up\_transaction()$: Whenever a Transaction terminates, id of that transaction will be removed from the $live\_trans\_list()$}
\begin{algorithmic}[1]
\STATE lock $live\_trans\_list()$;
\STATE $live\_trans\_list()\leftarrow (live\_trans\_list()-i)$;
\STATE unlock $live\_trans\_list()$;
\STATE return $(live\_trans\_list())$.
\end{algorithmic}
\end{algorithm}
}

\subsection{Proof of Garbage Collection}

We have the following useful lemma on garbage collection. 
\begin{lemma}
\label{lem:garbage-rule}
After garbage collection the new graph will be acyclic iff the original MVCG(V,E) will be acyclic.
\end{lemma}



